Information, Energy and Density for Ad Hoc Sensor Networks over Correlated Random Fields: Large Deviations Analysis

Using large deviations results that characterize the amount of information per node on a two-dimensional (2-D) lattice, asymptotic behavior of a sensor network deployed over a correlated random field for statistical inference is investigated. Under a 2-D hidden Gauss-Markov random field model with symmetric first order conditional autoregression, the behavior of the total information [nats] and energy efficiency [nats/J] defined as the ratio of total gathered information to the required energy is obtained as the coverage area, node density and energy vary.

==> setup.tex <==
\pagestyle{myheadings}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\setcounter{footnote}{1}
%\input /user/ltong/tex/macros/macros.tex
\makeatletter
\newdimen{\captionwidth}
\long\def\@makecaption#1#2{%
\captionwidth 1.0\hsize% use current value of \hsize
\vskip 10pt%
\setbox\@tempboxa\hbox{#1: #2}%
  \ifdim \wd\@tempboxa >\captionwidth%
    \setbox\@tempboxa\hbox{#1:\hspace*{.5em}}%
    \hfil\parbox{\captionwidth}{\raggedright\hangindent \wd\@tempboxa%
    \hangafter=1\unhbox\@tempboxa#2}\hfill%
%  \else \hbox to\captionwidth{\hfil\box\@tempboxa\hfil}%
  \else\centerline{\box\@tempboxa}%
  \fi
}
\makeatother
%\input epsf
\def\scalefig#1{\epsfxsize #1\textwidth}
\makeatletter
\font\hmed=cmr10 at 10pt
\def\ps@plain{\let\@mkboth\@gobbletwo
     \def\@oddhead{}\def\@oddfoot{\hmed\hfil
 / \footernote\ / \qquad \thepage}
\def\@evenhead{}\def\@evenfoot{\hmed
\thepage\qquad /  / \footernote\ \hfil }
}
\def\footernote{{\it \small }} 

\makeatother

\makeatletter
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{assumption}{A}
\newtheorem{properties}{Properties}
\newtheorem{conjecture}{Conjecture}
\newtheorem{criterion}{Criterion}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{notation}{Notation}
\newtheorem{derivation}{Derivation}
%\bibliographystyle{ieee}

\renewcommand\baselinestretch{1.0}

%\footernote{\protect\tiny Submitted to IEEE Transactions On Signal Processing}











